Towards a General Framework for Formal Reasoning about Java Bytecode Transformation

Program transformation has gained a wide interest since it is used for several purposes: altering semantics of a program, adding features to a program or performing optimizations. In this paper we focus on program transformations at the bytecode level. Because these transformations may introduce errors, our goal is to provide a formal way to verify the update and establish its correctness. The formal framework presented includes a definition of a formal semantics of updates which is the base of a static verification and a scheme based on Hoare triples and weakest precondition calculus to reason about behavioral aspects in bytecode transformation

==> eptcsdata.tex <==
\providecommand{\firstpage}{63}
\providecommand{\publicationstatus}{Adel Bouhoula, Tetsuo Ida and Fairouz Kamareddine (Eds.):\\
Symbolic Computation in Software Science 2012 (SCSS2012)\\
EPTCS 122, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.122.6}{10.4204/EPTCS.122.6}}
\pdfoutput=1

